How to Train BERT with an Academic Budget

While large language models a la BERT are used ubiquitously in NLP, pretraining them is considered a luxury that only a few well-funded industry labs can afford. How can one train such models with a more modest budget? We present a recipe for pretraining a masked language model in 24 hours using a single low-end deep learning server. We demonstrate that through a combination of software optimizations, design choices, and hyperparameter tuning, it is possible to produce models that are competitive with BERT-base on GLUE tasks at a fraction of the original pretraining cost.

==> tables/ablation_flops.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{p{3cm}  p{2cm} p{3cm} p{4cm}}
\toprule
&
\bf MLM 24hr & \bf Sentences/sec & \bf Flops in 22001 steps  \\
% \bf ppl \\
\midrule
24hr Calibrated   & 1.717 & 1088 & 1.40E+19 \\
\midrule
\textbf{-}Apex Layer Norm & 1.723 & 1053 & 1.40E+19 \\
\textbf{-}Sparse Output & 1.728 & 1052 & 1.54E+19 \\
\textbf{-}Fused linear \& Sparse Output & 1.732 & 1048 & 1.54E+19 \\
\midrule
\bertbase & 2.050 & - & 5.03E+18 \\
\bertlarge & 2.318 & - & 1.54E+19 \\
% \textbf{+}\textsc{DeepSpeed} Kernel & 1.696 & 1200 \\\midrule
% Intra-shard dup. & 1.783 & - \\\bottomrule
\end{tabular}
\caption{Ablation study of various pretraining techniques. Leftmost column: model attempted. The techniques specified with \textbf{-} were \textit{removed} from the calibrated version, and those with \textbf{+} were \textit{added}. }
\label{tab:ablation_flops}
\end{table*}


==> tables/best_glue_configurations.tex <==
\begin{table*}[t]
\centering
\small
\begin{tabular}{@{}lccccc@{}}
\toprule
\bf Hyperparameter  & \bf SST-2, MNLI, QNLI & \bf CoLA  & \bf RTE, STS-B, WNLI & \bf MRPC & \bf QQP \\
\midrule 
Learning Rate & 0.00008 & 0.00008 & 0.00008 & 0.00008 & 0.00008  \\
Batch Size & 32  & 32   & 16 & 16 & 32 \\
Max Epochs & 3  & 10  & 10   & 3    & 5 \\
Warmup Proportion & 0.06  & 0.06 & 0.06 & 0.06  & 0.06 \\
\bottomrule
\end{tabular}
\caption{
The best hyperparameter settings found for each GLUE task in the benchmark, when taking the median from 5 seeds per setup.
}
\label{tab:glue_hp_best_setup}
\end{table*}


% \toprule
% \bf Hyperparameter  & \bf Learning Rate & \bf Batch Size & \bf Warm-up ratio & \bf Max Epochs \\
% \midrule 
% RTE & 0.00008 & 16 & 0.06 & 10 \\
% SST-2 & 0.00008 & 32 & 0.06 & 3 \\
% MRPC & 0.00008 & 16  & 0.06 & 3 \\
% CoLA & 0.00008 & 32 & 0.06 & 10 \\
% STS-B & 0.00008 & 16 & 0.06 & 10 \\
% WNLI & 0.00008 & 16 & 0.06 & 10 \\
% MNLI & 0.00008 & 32 & 0.06 & 3 \\
% QQP & 0.00008 & 32 & 0.06 & 5 \\
% QNLI & 0.00008 & 32 & 0.06 & 3	 \\


==> tables/electra_comparison.tex <==
\begin{table}[t]
\centering
\small
\begin{tabular}{ccc}
\toprule
\textbf{Examples} &
\bf \textit{Without} Prompt &
\bf \textit{With} Prompt \\
\midrule
32 & 0.511 & 0.806 \\
64 & 0.554 & 0.811 \\
128 & 0.800 & 0.853 \\
256 & 0.834 & 0.860 \\
512 & 0.849 & 0.872 \\
1024 & 0.863 & 0.881 \\
\bottomrule
\end{tabular}
\caption{\textcolor{red}{Results for 24hBERT on the SST-2 task with and without prompts in the few-shot setting (5 seeds for each \#examples, with 25\% of them used for validation).}\peter{perhaps convert to figure}}
\label{tab:electra_comp}
\end{table}


==> tables/mlm_24_versus_metrics.tex <==
\begin{figure}
\centering
  \includegraphics[width=\columnwidth]{images/MNLI vs MLM 24hr.pdf}
%   \vspace{-15pt}
\caption{plotting the top MNLI accuracy relative to the MLM validation loss at the 24 hours }
  \label{fig:24hr_vs_mnli}
\end{figure}

\begin{figure}
\centering
  \includegraphics[width=\columnwidth]{images/MLM 24hr vs MLM 12hr.pdf}
%   \vspace{-15pt}
\caption{plotting the MLM validation loss at the 12 hours mark relative to the 24 hour mark. As expected, there is a positive correlation (87.22\% with Pearson correlation) between both values. }
  \label{fig:24hr_vs_12hr}
\end{figure}

==> tables/mnli_trick.tex <==
\begin{table}[t]
\centering
\small
\begin{tabular}{@{}lcccc@{}}
\toprule
& \bf RTE & \bf MRPC & \bf STS-B  \\ % & \bf Avg.
% \#Examples & 2.5k & 3.7k & 7k  \\
\midrule 
\textbf{24hBERT}       & 75.3 & 88.5 & 86.8  \\ % & 81.1
\bertbase              & 76.5 & 89.9 & 87.7  \\ % & 81.5
\bertlarge             & 78.3 & 89.9 & 87.5  \\ % & 83.0
\robertabase           & 79.6 & 89.7 & 88.3  \\ % & 83.4
\bottomrule
\end{tabular}
\caption{Performance on GLUE test sets, when finetuning each model using the MNLI dataset first.}
% , and then performing additional fine-tuning on RTE, MRPC, and STS-B.  

\label{tab:glue_tasks_mnli}
\end{table}


==> tables/other_languages_results.tex <==
\begin{table}[t]
\centering
\small
\begin{tabular}{@{}lc@{}}
\toprule
& \bf XNLI French  \\
% \#Examples & 392k   \\
\midrule 
\camembase     & 79.1  \\
24hBERT        & 78.5  \\
\bottomrule
\end{tabular}
\caption{Performance on the XNLI French development set. \peter{perhaps merge this table with Table 4? add a new col and a row for Camembert}}
\label{tab:other_lang_tasks}
\end{table}

% Performance on the XNLI French validation set. The results for each model are the median result, using 5 seeds, applied with the best finetuning setup per model.
%  The results shown are the best hyperparameter configuration of 5 random seeds.

